Weighted Pseudorandom Generators for Read-Once Branching Programs via Weighted Pseudorandom Reductions

We study weighted pseudorandom generators (WPRGs) and derandomizations for read-once branching programs (ROBPs). Denote $n$ and $w$ as the length and the width of a ROBP. We have the following results. For standard ROBPs, we give an explicit $\varepsilon$-WPRG with seed length $$O\left(\frac{\log n\log (nw)}{\max\left\{1,\log\log w-\log\log n\right\}}+\log w \left(\log\log\log w-\log\log\max\left\{2,\frac{\log w}{\log \frac{n}{\varepsilon}}\right\}\right)+\log\frac{1}{\varepsilon}\right).$$ For permutation ROBPs with unbounded widths and single accept nodes, we give an explicit $\varepsilon$-WPRG with seed length $$O\left( \log n\left( \log\log n + \sqrt{\log(1/\varepsilon)} \right)+\log(1/\varepsilon)\right). $$ We also give a new Nisan-Zuckerman style derandomization for regular ROBPs with width $w$, length $n = 2^{O(\sqrt{\log w})}$, and multiple accept nodes. We attain optimal space complexity $O(\log w)$ for arbitrary approximation error $\varepsilon = 1/\text{poly} (w)$. All our results are based on iterative weighted pseudorandom reductions, which can iteratively reduce fooling long ROBPs to fooling short ones.

==> figures/derandomization_alg.tex <==
\begin{tikzpicture}

    % Define layer height
    \def\layerheight{1}
    

    % Layer 2: Two rectangles of different widths
    \draw[fill=red!20] (0, 3*\layerheight) rectangle (0.6*0.9*\textwidth, 4*\layerheight);
    \node at (0.3*0.9*\textwidth, 3.5*\layerheight) {$\Rot_{\widetilde{G}^{(2)}_{0\to 1}}$};
    \draw[fill=green!20] (0.6*0.9*\textwidth, 3*\layerheight) rectangle (0.9*\textwidth, 4*\layerheight);
    \node at (0.8*0.9*\textwidth, 3.5*\layerheight) {$\Rot_{\widetilde{G}^{(2)}_{1\to 2}}$};
    
    % Layer 3: 3 rects under the first rect of layer 2, 2 under the second
    \draw[fill=yellow!30] (0, 2*\layerheight) rectangle (0.2*0.9*\textwidth, 3*\layerheight);
    \node at (0.1*0.9*\textwidth, 2.5*\layerheight) {$\Rot_{\widetilde{G}^{(1)}_{0\to 1}}$};
    \draw[fill=yellow!30] (0.2*0.9*\textwidth, 2*\layerheight) rectangle (0.4*0.9*\textwidth, 3*\layerheight);
    \node at (0.3*0.9*\textwidth, 2.5*\layerheight) {$\Rot_{\widetilde{G}^{(1)}_{1\to 2}}$};
    \draw[fill=yellow!30] (0.4*0.9*\textwidth, 2*\layerheight) rectangle (0.6*0.9*\textwidth, 3*\layerheight);
    \node at (0.5*0.9*\textwidth, 2.5*\layerheight) {$\Rot_{\widetilde{G}^{(1)}_{2\to 3}}$};
    \draw[fill=orange!40] (0.6*0.9*\textwidth, 2*\layerheight) rectangle (0.8*0.9*\textwidth, 3*\layerheight);
    \node at (0.7*0.9*\textwidth, 2.5*\layerheight) {$\Rot_{\widetilde{G}^{(1)}_{3\to 4}}$};
    \draw[fill=orange!40] (0.8*0.9*\textwidth, 2*\layerheight) rectangle (0.9*\textwidth, 3*\layerheight);
    \node at (0.9*0.9*\textwidth, 2.5*\layerheight) {$\Rot_{\widetilde{G}^{(1)}_{4\to 5}}$};
    
    % Layer 5: Row of small rectangles joined by dots
    \foreach \x in {0.1, 0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8, 0.9, 1} {
        \draw[fill=purple!20] (\x*0.9*\textwidth-0.1*0.9*\textwidth, 1*\layerheight) rectangle (\x*0.9*\textwidth, 2*\layerheight);
        
    };
    \foreach \x in {0.1, 0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8, 0.9, 1} {
        %\draw[->, -latex, out=330, in=21] (\x * 0.9*\textwidth-0.1*0.9*\textwidth, \layerheight) to (\x * 0.9*\textwidth, 1*\layerheight);
        \draw[->, -latex] (\x * 0.9*\textwidth-0.1*0.9*\textwidth, \layerheight) to (\x * 0.9*\textwidth, 1*\layerheight);
        }
        
    \foreach \x in {1,2,3,4,5,6,7,8,9,10} {
        \pgfmathsetmacro{\y}{\x-1}
        \node at (\x*0.9*\textwidth/10-0.05*0.9*\textwidth, 1.5*\layerheight) {$\Rot_{\widetilde{G}^{(0)}_{\pgfmathprintnumber{\y}\to \x}}$};
    }

    \foreach \x in {0.1, 0.3, 0.5, 0.7, 0.9} {
        \draw[->, -latex] (\x * 0.9*\textwidth, 0.6*\layerheight) to (\x * 0.9*\textwidth, 1*\layerheight);
        \node at (\x*0.9*\textwidth, 0.4*\layerheight) {$\Rot_{\widetilde{H}^{(0)}_1}$};
    }

    \foreach \x in {0.2,0.8} {
        \draw[->, -latex] (\x * 0.9*\textwidth, 0.2*\layerheight) to (\x * 0.9*\textwidth, 1*\layerheight);
        \node at (\x*0.9*\textwidth, 0*\layerheight) {$\Rot_{\widetilde{H}^{(1)}_1}$};
    }

    \foreach \x in {0.4} {
        \draw[->, -latex] (\x * 0.9*\textwidth, 0.2*\layerheight) to (\x * 0.9*\textwidth, 1*\layerheight);
        \node at (\x*0.9*\textwidth, 0*\layerheight) {$\Rot_{\widetilde{H}^{(1)}_2}$};
    }

     \foreach \x in {0.6} {
        \draw[->, -latex] (\x * 0.9*\textwidth, -0.2*\layerheight) to (\x * 0.9*\textwidth, 1*\layerheight);
        \node at (\x*0.9*\textwidth, -0.4*\layerheight) {Use the next seed $x^{(2)}_2$};
    }
     \foreach \x in {0.0} {
        \draw[->, -latex] (\x * 0.9*\textwidth, -0.2*\layerheight) to (\x * 0.9*\textwidth, 1*\layerheight);
        \node at (\x*0.9*\textwidth, -0.4*\layerheight) {Use seed $x^{(2)}_1$};
    }

    

    
    \end{tikzpicture}
